Reality3DSketch: Rapid 3D Modeling of Objects from Single Freehand Sketches

The emerging trend of AR/VR places great demands on 3D content. However, most existing software requires expertise and is difficult for novice users to use. In this paper, we aim to create sketch-based modeling tools for user-friendly 3D modeling. We introduce Reality3DSketch with a novel application of an immersive 3D modeling experience, in which a user can capture the surrounding scene using a monocular RGB camera and can draw a single sketch of an object in the real-time reconstructed 3D scene. A 3D object is generated and placed in the desired location, enabled by our novel neural network with the input of a single sketch. Our neural network can predict the pose of a drawing and can turn a single sketch into a 3D model with view and structural awareness, which addresses the challenge of sparse sketch input and view ambiguity. We conducted extensive experiments synthetic and real-world datasets and achieved state-of-the-art (SOTA) results in both sketch view estimation and 3D modeling performance. According to our user study, our method of performing 3D modeling in a scene is $>$5x faster than conventional methods. Users are also more satisfied with the generated 3D model than the results of existing methods.

==> table/table5.tex <==
% %% table 1
% \begin{table*}[ht]
% \begin{center}
% \caption{{{The quantitative evaluation of sketch-view estimation}}
% \scalebox{1}{

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

% \hline
% \multicolumn{15}{|c|}{Shapenet-synthetic (MAE $\downarrow)$} \\
% \hline
%  & car & sofa & airplane & bench & display & chair & table  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean\\
% \hline
% Sketch2Model & 1.0751 & 1.5989 & 2.3899 & 1.8345 & 1.8944 & 1.8690 & 1.2857 & 2.2732 & 1.2148 & 2.4303 & 3.6884 & 4.4071 & 3.3226 & 2.2526 \\
% Ours & 0.746 & 0.620 & 0.618 & 0.477 & 0.550 & 0.515 & 0.470 & 0.673 & 0.667 & 0.624 & 0.569 & 0.463 & 0.606 & 0.584 \\
% \hline
% \textbf{Ours (GT Pos)} & \textbf{0.796} & \textbf{0.651} & \textbf{0.644} & \textbf{0.500} & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} & \textbf{0.738} & \textbf{0.705} & \textbf{0.651} & \textbf{0.595} & \textbf{0.469} & \textbf{0.619} & \textbf{0.618} \\
% \textbf{Ours (Pred Pos)} & 0.793 & 0.649 & 0.641 & \textbf{0.500} & 0.583 & 0.541 & 0.504 & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & \textbf{0.619} & 0.604\\
% \hline
% \end{tabular}}
% \end{center}

% \label{table:table1}

% \end{table*}

%% table 1
\begin{table*}[ht]
\begin{center}
\caption{{{The quantitative evaluation of sketch-view estimation}}
\scalebox{1}{

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\hline
\multicolumn{15}{|c|}{Shapenet-synthetic (MAE $\downarrow)$} \\
\hline
 & car & sofa & airplane & bench & display & chair & table  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean\\
\hline
Sketch2Model & 1.0751 & 1.5989 & 2.3899 & 1.8345 & 1.8944 & 1.8690 & 1.2857 & 2.2732 & 1.2148 & 2.4303 & 3.6884 & 4.4071 & 3.3226 & 2.2526 \\
Ours & 0.746 & 0.620 & 0.618 & 0.477 & 0.550 & 0.515 & 0.470 & 0.673 & 0.667 & 0.624 & 0.569 & 0.463 & 0.606 & 0.584 \\
\hline
\textbf{Ours (GT Pos)} & \textbf{0.796} & \textbf{0.651} & \textbf{0.644} & \textbf{0.500} & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} & \textbf{0.738} & \textbf{0.705} & \textbf{0.651} & \textbf{0.595} & \textbf{0.469} & \textbf{0.619} & \textbf{0.618} \\
\textbf{Ours (Pred Pos)} & 0.793 & 0.649 & 0.641 & \textbf{0.500} & 0.583 & 0.541 & 0.504 & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & \textbf{0.619} & 0.604\\
\hline
\end{tabular}}
\end{center}

\label{table:table1}

\end{table*}

==> table/table7.tex <==
%% table 4
\begin{table*}[h]
\begin{center}
\caption{The sensitivity analysis for sampling different number of silhouettes}
\scalebox{1}{

\begin{tabular}{|c|c|ccccccc|}
\hline
\multicolumn{8}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow)$} \\

\hline
                partial level & method      & airplane       & bench          & cabinet        & car            & chair          & lamp           & rifle          \\ \hline
\multirow{2}{*}{0}  & sketch2model & 0.624          & 0.481          & \textbf{0.701} & 0.751          & 0.522          & \textbf{0.472} & 0.612          \\
                    & ours         & \textbf{0.632} & \textbf{0.510} & 0.692          & \textbf{0.782} & \textbf{0.526} & 0.467          & \textbf{0.631} \\ \hline
\multirow{2}{*}{10} & sketch2model & 0.560          & 0.454          & \textbf{0.675} & 0.695          & 0.483          & \textbf{0.445} & 0.565          \\
                    & ours         & \textbf{0.578} & \textbf{0.476} & 0.663          & \textbf{0.743} & \textbf{0.486} & 0.442          & \textbf{0.595} \\ \hline
\multirow{2}{*}{20} & sketch2model & 0.481          & 0.419          & \textbf{0.638} & 0.619          & \textbf{0.434} & \textbf{0.403} & 0.505          \\
                    & ours         & \textbf{0.506} & \textbf{0.438} & 0.635          & \textbf{0.689} & 0.432          & 0.402          & \textbf{0.543} \\ \hline
               partial level & method         & sofa           & table          & telephone      & watercraft     & diplay         & loudspeaker    & mean           \\ \hline
\multirow{2}{*}{0}  & sketch2model & 0.622          & 0.478          & 0.719          & \textbf{0.586} & \textbf{0.604} & \textbf{0.641} & 0.601          \\
                    & ours         & \textbf{0.640} & \textbf{0.510} & \textbf{0.758} & 0.584          & 0.589          & 0.631          & \textbf{0.611} \\ \hline
\multirow{2}{*}{10} & sketch2model & 0.580          & 0.437          & 0.704          & \textbf{0.549} & \textbf{0.573} & \textbf{0.628} & 0.565          \\
                    & ours         & \textbf{0.604} & \textbf{0.465} & \textbf{0.733} & 0.547          & 0.552          & 0.614          & \textbf{0.576} \\ \hline
\multirow{2}{*}{20} & sketch2model & 0.516          & 0.400          & 0.682          & 0.489          & \textbf{0.525} & \textbf{0.606} & 0.517          \\
                    & ours         & \textbf{0.550} & \textbf{0.425} & \textbf{0.711} & \textbf{0.499} & 0.499          & 0.595          & \textbf{0.532} \\ \hline
\end{tabular}}
\end{center}

\label{table:tablevii}

\end{table*}

